Dual Contrastive Learning for Unsupervised Image-to-Image Translation

Unsupervised image-to-image translation tasks aim to find a mapping between a source domain X and a target domain Y from unpaired training data. Contrastive learning for Unpaired image-to-image Translation (CUT) yields state-of-the-art results in modeling unsupervised image-to-image translation by maximizing mutual information between input and output patches using only one encoder for both domains. In this paper, we propose a novel method based on contrastive learning and a dual learning setting (exploiting two encoders) to infer an efficient mapping between unpaired data. Additionally, while CUT suffers from mode collapse, a variant of our method efficiently addresses this issue. We further demonstrate the advantage of our approach through extensive ablation studies demonstrating superior performance comparing to recent approaches in multiple challenging image translation tasks. Lastly, we demonstrate that the gap between unsupervised methods and supervised methods can be efficiently closed.

==> figs/resultmore.tex <==
\begin{figure}[htb]
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \text{\small Input}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \text{\small DCLGAN}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
      \text{\small SimDCL}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
        \text{\small CUT}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
        \text{\small CycleGAN}
  \end{minipage} 
  \\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input1.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl1.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim1.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut1.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle1.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input2.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl2.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim2.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut2.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle2.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input3.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl3.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim3.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut3.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle3.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input4.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl4.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim4.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut4.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle4.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input5.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl5.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim5.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut5.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle5.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input6.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl6.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim6.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut6.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle6.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input7.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl7.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim7.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut7.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle7.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input8.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl8.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim8.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut8.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle8.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input9.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl9.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim9.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut9.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle9.png}
  \end{minipage} 
\\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input10.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl10.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim10.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut10.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle10.png}
  \end{minipage} 
  \\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input11.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl11.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim11.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut11.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle11.png}
  \end{minipage} 
  \\
  \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/input12.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/dcl12.png}
  \end{minipage} 
      \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/sim12.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cut12.png}
  \end{minipage} 
    \begin{minipage}[t]{0.19\linewidth} 
    \centering 
    \includegraphics[width=0.6in, height=0.6in]{ figs/result3/cycle12.png}
  \end{minipage} 
  \caption{Second stage: Comparison between the best four methods on five more tasks including Zebra $\rightarrow$ Horse, Van Gogh $\rightarrow$ Photo, Dog $\rightarrow$ Cat, Label $\rightarrow$ Facade, and Orange $\rightarrow$ Apple. We randomly pick two samples for each task. Our DCLGAN performs both geometry changes and texture changes. The last two rows show two typical failure cases, the first one fails to translate since input is only a small part of zebra, the last one fails to keep the structure of humans, translating them to mountains.}
  \label{fig:second}
\end{figure}

==> figs/supp1.tex <==
\begin{figure*}[htb]
  \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \text{Input}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \text{DCLGAN}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
      \text{Variant}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
        \text{Label}
  \end{minipage} 
  \\
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/input0.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/122_A.png}
  \end{minipage} 
      \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/va0.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/label0.png}
  \end{minipage} 
  \\
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/input1.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/dcl1.png}
  \end{minipage} 
      \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/va1.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/label1.png}
  \end{minipage} 
  \\
      \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/input2.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/dcl2.png}
  \end{minipage} 
      \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/va2.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/label2.png}
  \end{minipage} 
  \\
      \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/input3.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/191_A.png}
  \end{minipage} 
      \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/va3.png}
  \end{minipage} 
    \begin{minipage}[t]{0.245\linewidth} 
    \centering 
    \includegraphics[width=1.65in, height=1in]{ figs/supp1/label3.png}
  \end{minipage} 
 \caption{Comparison between DCLGAN and variant drawing external negatives on task CityScapes.}
  \label{fig:supp1}
\end{figure*}

==> figs/supp2.tex <==
\begin{figure*}[htb]
  \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \text{Input}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \text{DCLGAN}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
      \text{Variant}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
        \text{Input}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \text{DCLGAN}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
      \text{Variant}
  \end{minipage}   
  \\
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/input4.png}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/dcl4.png}
  \end{minipage} 
      \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/va4.png}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/input5.png}
  \end{minipage} 
     \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/dcl5.png}
  \end{minipage} 
      \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/va5.png}
  \end{minipage} 
    \\
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/input6.png}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/dcl6.png}
  \end{minipage} 
      \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/va6.png}
  \end{minipage} 
    \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/input7.png}
  \end{minipage} 
     \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/dcl7.png}
  \end{minipage} 
      \begin{minipage}[t]{0.163\linewidth} 
    \centering 
    \includegraphics[width=1.1in, height=1.1in]{ figs/supp1/va7.png}
  \end{minipage} 
 \caption{Comparison between DCLGAN and variant drawing external negatives on tasks Horse $\rightarrow$ Zebra and Zebra $\rightarrow$ Horse. }
  \label{fig:supp2}
\end{figure*}
